On gauge theory and parallel transport in principal 2-bundles over Lie groupoids

We investigate an interplay between some ideas in traditional gauge theory and certain concepts in fibered categories. We accomplish this by introducing a notion of a principal Lie 2-group bundle over a Lie groupoid and studying its connection structures, gauge transformations, and parallel transport. We obtain a Lie 2-group torsor version of the one-one correspondence between fibered categories and pseudofunctors. This results in a classification of our principal 2-bundles based on their underlying fibration structures. This allows us to extend a class of our principal 2-bundles to be defined over differentiable stacks presented by the base Lie groupoids. We construct a short exact sequence of VB-groupoids, namely, the 'Atiyah sequence' associated to our principal 2-bundles. Splitting and splitting up to a natural isomorphism of our Atiyah sequence, respectively, gives us notions of 'strict connections' and 'semi-strict connections' on our principal 2-bundles. We describe such connections in terms of Lie 2-algebra valued 1-forms on the total Lie groupoids. The underlying fibration structure of our 2-bundle provides an existence criterion for strict and semi-strict connections. We study the action of the 2-group of gauge transformations on the groupoid of strict and semi-strict connections, and interestingly, we observe an extended symmetry of semi-strict connections. We demonstrate an interrelationship between `differential geometric connection-induced horizontal path lifting property in traditional principal bundles' and the `category theoretic cartesian lifting of morphisms in fibered categories' by developing a theory of connection-induced parallel transport along a particular class of Haefliger paths in the base Lie groupoid of our principle 2-bundles. Finally, we employ our results to introduce a notion of parallel transport along Haefliger paths in the setup of VB-groupoids.

==> Title.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%title page
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{pdfpages}
\thispagestyle{empty}
\begin{center}{
\textbf{\LARGE{Stochastic Analysis of Nematic Liquid Crystals and Related Physical Models}}
}
\end{center}{ \par}

\vspace*{\fill}

\bigskip{}
\begin{center}{
{\it {\large A thesis submitted for the degree of}}\\
\vspace {0.5cm}
{{\Large\bf Doctor of Philosophy}}\\
\vspace {0.5cm}
{\it {\large in the}}\\
\vspace {0.5cm} {\bf {\Large School of Mathematics}}}
\end{center}
\vspace*{\fill}
\begin{center}
%{\it By}\\
\end{center}
\vspace*{\fill}
\begin{center}{\textbf{\Large {\bf Akash Ashirbad Panda}}}\end{center}{\Large \par}

\vspace*{\fill}

\begin{center}
\includegraphics[scale=0.5]{11.jpg}{\small}\\
{\small SCHOOL OF MATHEMATICS}\\
{\small INDIAN INSTITUTE OF SCIENCE EDUCATION AND RESEARCH}\\
{\small THIRUVANANTHAPURAM - 695551}\\
{\small INDIA}\end{center}{\small
\par}

\begin{center}{\small August 2019}\end{center}{\small \par}
\clearpage
%--------------------------------------------------------------------------
%backside of the front cover
\newpage
\thispagestyle{empty}
\bigskip{}
\vspace{1cm} \cleardoublepage
%\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%DECLARATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\thispagestyle{plain}
\begin{center}\textbf{\huge Declaration}\end{center}{\huge \par}
%\bigskip{}
\vspace{1cm} I hereby declare that the work reported in this thesis
is original and was carried out by me during my tenure as a PhD
student at the \textbf{School of Mathematics, Indian Institute of
Science Education and Research Thiruvananthapuram}. Such material as
has
been obtained from other sources has been duly acknowledged in the thesis.\\

\vspace{1in} \noindent Place: IISER Thiruvananthapuram\hfill {\bf
Akash Ashirbad Panda}\\\smallskip Date\ : August 2019 \hfill
\\\smallskip

\vspace{1cm}



\noindent
{\bf Certified} that the work incorporated in the thesis

\vspace{0.1cm}

\begin{center} {\bf ``Stochastic Analysis of Nematic Liquid Crystals and Related Physical Models"}
\end{center}

\vspace{0.1cm}

\noindent submitted by {\bf Akash Ashirbad Panda} was carried out by the
candidate under my supervision. This thesis has not formed the basis
for the award of any degree, of any university or institution.

\vspace{1in} \noindent Place: IISER Thiruvananthapuram\hfill {\bf
Dr. Utpal Manna}\\ \smallskip Date\ : August 2019 \hfill(Thesis supervisor)\\
\smallskip
%}
%------------------------------------------------------------------------------
\newpage
\thispagestyle{empty}
\cleardoublepage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Dedication
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %blank chapter, no title, not included in table of contents
%\thispagestyle{empty} %no page number
%\addtocounter{page}{-1} %ignore this page when counting
%\vspace{2.5in} %start the dedication halfway down
%\begin{center} %center everything
%\textit{\huge Dedication (omit if not necessary)} %the wonderful words
%\end{center}
%------------------------------------------------------------------------------
%\newpage
%\thispagestyle{empty}
%\cleardoublepage
%\fi
\iffalse
\thispagestyle{empty}
\begin{figure}[c]
\begin{center}
\includegraphics[width=1.1\textwidth]{Manil.pdf}
\end{center}
\end{figure}
\clearpage
\newpage
\thispagestyle{empty}
\bigskip{}
\vspace{1cm} \cleardoublepage \fi



\thispagestyle{empty}
\begin{figure}%[c]
\begin{center}
\includegraphics[width=1\textwidth]{style2.pdf}
\end{center}
\end{figure}
\clearpage
\newpage
\thispagestyle{empty}
\bigskip{}
\vspace{1cm} \cleardoublepage
%\includepdf[pages={1}]{style.pdf}



\iffalse \thispagestyle{empty} \vspace*{\fill}
\begingroup
\begin{center}
\centering {\Huge {\chancery Dedicated to my family for their
endless love, care and support}}
\end{center}
\endgroup
\vspace*{\fill} \clearpage
\newpage
\thispagestyle{empty}
\bigskip{}
\vspace{1cm} \cleardoublepage \fi



\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Acknowledgements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\thispagestyle{plain}
\begin{center}\textbf{\Huge Acknowledgements}\end{center}{\huge \par}
\bigskip{}
%\vspace{0.5cm}
Undertaking this PhD has been a truly life-changing experience for
me and it would not have been possible without the support and
guidance that I received from my well wishers, friends, colleagues
and various institutions, to only some of whom it is possible to
give particular mention here.

First and foremost, I would like to express my deeply-felt thanks to
my supervisor, Dr. Utpal Manna for his patience, motivation,
enthusiasm, and immense knowledge. It has been a great honor for me
to be his first PhD student. Under his guidance I successfully
overcame many difficulties and learned deep mathematical theories in
this field. His advice on my research as well as on my career have
been invaluable. As my supervisor, he has constantly forced me to
remain focused on achieving my goal. His observations and comments
helped me to establish the overall direction of the research and to
move forward with investigation in depth.

I am extremely indebted to my institute Indian Institute of Science
Education and Research Thiruvananthapuram (IISER-TVM) for providing
necessary infrastructure and resources to accomplish my research
work. I thank my doctoral committee members Dr. Sreedhar B. Dutta,
Dr. M. P. Rajan, Dr. Anil Shaji and Dr. Dharmatti Sheetal for their
helpful suggestions and guidance throughout my PhD tenure. I would
like to extend my sincere thanks to Prof. E. D. Jemmis, former
Director, IISER-TVM (Professor, IISc Bangalore), Prof. V.
Ramakrishnan, Director, IISER-TVM, Prof. K. George Thomas, Dean,
IISER-TVM and  Dr. Joy Mitra, PhD co-ordinator, IISER-TVM for all
the advice and extensive support. I express my gratitude to all my
PhD course instructors. I am very much thankful to all the faculty
members and students of School of Mathematics, IISER-TVM for their
invaluable support and help throughout my stay at IISER-TVM.

I would like to sincerely acknowledge the Council of Scientific and
Industrial Research (CSIR), Government of India, New Delhi for
providing financial assistance in the form of Junior and Senior
Research Fellowship which supported me to perform my work
comfortably.

It has been a great honor for me to collaborate with Prof. S. S.
Sritharan, Naval Postgraduate School, Monterey, USA and his truly
inspiring teaching turned me towards writing my thesis in logic. I
am extremely grateful to Prof. P. Sundar, Louisiana State
University, USA for helpful discussions on exponential stability and
invariant measure during the ICTS winter school, December 2012 at
IISER-TVM.

I take this opportunity to remember and thank my M. Sc. teachers
Mrs. K. L. Anandavally, Dr. V. Madhukar Mallayya and Dr. James
Alexander at Mar Ivanios College, TVM for their continuous support
and care. I gratefully acknowledge K. V. Baiju, Govt. Women's
college, TVM for his encouragemnet and personal attention which have
provided a good and smooth basis for my PhD tenure. I also extend my
sincere gratitude towards all the Mathematics faculty members of Mar
Ivanios College, TVM, Mahatma Gandhi College, TVM and University
College, TVM for their blessings. I would like to express my
heartfelt gratitude to Late Prof. S. Unnithan, Dr. K. R. Arun and
Dr. Prakash Rajendran for their invaluable support and encouragement
during my teaching assistantship with them at IISER-TVM. My
successful completion of the thesis could not have been possible
without the endless support of Dr. P. Sainul Abideen, B. V. Ramesh,
K. S. G. Kurup, V. J. Divya, Jayaraj, Mini, Nafeesa, Nimmy, Praveen
Lal, Sreekumar, Suja, Vijesh, Vivek  at IISER-TVM. I would like to
thank all academic, administrative and technical staff members of
IISER-TVM who have been kind enough to advise and help in their
respective roles.

This acknowledgment would not be completed without mentioning my
friends at IISER-TVM who have given immense support, help and
encouragement at different stages of my stay at IISER-TVM.  I am
very much grateful to my ``sister" Chithra H. Sharma who helped me
in numerous ways during various stages of my PhD tenure. She was
always beside me during the happy and hard moments to push me and
motivate me. Thank you doesn't seem sufficient but it is said with
appreciation and respect to you for your support, encouragement,
care, understanding and precious friendship. It is also a great
pleasure for me to mention my good friends, Shyama, Nijamudheen,
Vishnu and Ajith for their love, care, support and creating a
pleasant atmosphere for me here. I would like to specially mention
the endless support and help by  Alex, Anoop Thomas, Atchutharao,
Baiju, Balu, Damodar Reddy, Debopriya Mukherjee, Deepthi Jose,
Deepesh, Gireesh, Haris, Jaise Jose,  Jissy, Joshya Shyamala,
Jyothish, Mayank,  Niyas Rehman, Pradeep, Priya Kumari,  Reshmi
Thomas, Rijo, Rohini, Sankaran Nampoothiri, Santhosh Kumar, Sabnam,
Shinaj, Sreerekha, Subila,  Vinayak Jagadish, Vidya, Vidyasagar. A
special thanks to Alex for helping me in drawing the figures needed
for the thesis. I take this opportunity to thank my BS-MS students
Ajai, Ajeesh, Atul Mohan, Athul Sivan, Jery Joy, Jimmy Joy,
Nagarjuna Mahadas, Pooja Agarwal, Salini Nair, Sarang Som, Sujeesh,
Srikanth, Srinath, Vrinda, Yadu Krishnan for their invaluable care
and love. A special thanks to Alex for helping me in drawing the
figures needed for the thesis. I am also thankful to all my PhD
friends and BS-MS students at IISER-TVM for their love, care and
encouragement. Apart from my friends at IISER-TVM, I expand my
sincere thanks to my friends Anoop, Arati, Bijo, Deepu, Jose,
Jothish, Ratheesh, Shanu, Sumith for their constant moral support
and prayers.

Last, but not least, I would like to dedicate this thesis to my
family and I would like to express my deepest gratitude to my
parents Mr. K. Mohanan and Mrs. K. Thankamany, for their love, moral
support, patience and sincere encouragement. My hard-working parents
have sacrificed their lives for my brother and myself. I am grateful
to my dad for giving me the life I ever dreamed. I can't express my
gratitude for my mom in words, whose unconditional love and care has
been my greatest strength. I would like to thank my younger brother
Mr. Maneesh T. Mohan and my sister in law Mrs. Thanima Maneesh for
their constant love and encouragement. Besides this, several people
have knowingly and unknowingly helped me in the successful
completion of this thesis. I would therefore like to offer my
sincere thanks to all of them.

I praise God, the almighty for having made everything possible by
giving me strength and courage to complete this thesis.

\cleardoublepage

%------------------------------------------------------------------------------
\newpage
\thispagestyle{empty} \cleardoublepage \fi





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Acknowledgements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\thispagestyle{plain}
\begin{center}\textbf{\Huge {\chancery Acknowledgements}}\end{center}{\huge \par}
\bigskip{}
\vspace{0.5cm}
%{\large {\chancery  \\
%\quad \\ \quad \\ \indent\qquad\qquad\qquad\qquad\qquad\qquad\qquad
%\qquad\qquad\qquad\qquad\quad Akash Ashirbad Panda}}
{\Large {\chancery
This thesis is the culmination of my journey of Ph.D which was just like climbing a high peak step by step
accompanied with encouragement, hardship, trust, and frustration. When I found myself at top experiencing
the feeling of fulfillment, I realized though only my name appears on the cover of this thesis, a great
many people including my family members, well-wishers, my teachers, my friends, colleagues and various institutions have
contributed to accomplish this huge task. 

At this moment of accomplishment I am greatly indebted to my research guide
Dr. Utpal Manna for introducing me to this exciting field of mathematics and for his
dedicated help, advice, inspiration, encouragement and continuous support,
throughout my Ph.D. His enthusiasm, integral view on research and his mission for
providing high-quality work, has made a deep impression on me. During our course
of interaction during the last four years, I have learnt extensively from him,
including how to raise new possibilities, how to regard an old question from a new
perspective, how to approach a problem by systematic thinking. I am really glad to be associated with a person like Dr. Utpal Manna in my life. I could not have imagined having a better advisor and mentor for my Ph.D study.

My special words of thanks should also go to our collaborator Prof. Zdzis\l aw Brze\'zniak for his continuous support, guidance, cooperation and encouragement. He is a very enthusiastic researcher and an exceptional teacher. He has been pivotal to this thesis. I have not only learnt mathematics from him but also, how to be
a good teacher and researcher. I owe him lots of gratitude for having me shown
the actual way of research. I thank him for giving his precious time to me in his busy schedule. I would like to express my sincere gratitude to him for countless values that were instilled in me during my short stays in York, UK. Also I would like to thank our collaborator Paul Razafimandimby for his time and valuable inputs in my research works. 

I am extremely indebted to my institute, Indian Institute of Science
Education and Research Thiruvananthapuram (IISER-TVM) for providing
necessary infrastructure and resources to accomplish my research
work. I thank my doctoral committee members Dr. Dharmatti Sheetal,
Dr. K. R. Arun and Dr. P. Devaraj for their
helpful suggestions and guidance throughout my PhD tenure. I would
like to extend my sincere thanks to Prof. E. D. Jemmis former
Directors, IISER-TVM (Professor, IISc Bangalore), Prof. V.
Ramakrishnan, former
Director, IISER-TVM and Prof. J. N. Moorthy Director, IISER-TVM, for all
the extensive support. I express my gratitude to all my
masters course instructors. I am very much thankful to all the faculty
members and students of School of Mathematics, IISER-TVM for their
invaluable support and help throughout my stay at IISER-TVM.

I would like to mention ``The Royal Society International Exchanges award IE140328" led by Professor Zdzis\l aw Brze\'zniak at the University of York, UK and Dr. Utpal Manna at IISER Thiruvananthapuram. I would like to thank all academic,
administrative and technical staff members of IISER-TVM as well as of University of York who have
been kind enough to advise and help in their respective roles.

This acknowledgment would not be completed without mentioning my
friends at IISER-TVM who have given immense support, help and
encouragement at different stages of my stay at IISER-TVM. I would like to
specially mention the endless support and help by Arun Maurya, Ammu, Tania, Mahendra, Vatsal, Atmaram, Sharvari, Adittya and all other Mathematics Ph.Ds. A special thanks to my senior and a close friend Debopriya for her constant moral support, invaluable care and love. Also I would like to thank my senior Dr. Manil T Mohan for his valuable advises. I would like to specially mention the selfless care, encouragement and life values given by my dear friend Saurav. Particularly, I would like to mention the constant moral support and motivation of my friends Abhraneel, Brijesh, Pramod and Hareram. I would like to thank all of my Integrated PhD batchmates who joined IISER-TVM in 2013. I would like to commend Nimit bhaiya and Gaurav bhaiya for their help while my stay in York. Apart from my friends at IISER-TVM, I expand my sincere thanks to my cricket playing mates and Odia speaking group
for teaching other aspects of my life.

Finally, I acknowledge the people who mean a lot to me, my parents, Mr. Ashok Kumar Panda and Mrs. Krushnapriya Panda, for showing faith in me
and giving me liberty to choose what I desired. I salute you all for the selfless love, care, pain and sacrifice you
did to shape my life. Although you hardly understood what I researched on, you were willing to support any
decision I made. I would never be able to pay back the love and affection showered upon by my parents. Also I would like to acknowledge my sister, Guli for her love and support for me. I would like to thank all of my family relatives for their love and support. As always it is impossible to mention everybody who had an impact to this work
however there are those whose spiritual support is even more important. I would therefore like to offer my sincere thanks to all of them.

I thank the Almighty for giving me the strength and patience to work through all these years so that today I
can stand proudly with my head held high.
}}
\cleardoublepage

%------------------------------------------------------------------------------
\newpage
\thispagestyle{empty} \cleardoublepage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Preface
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\pagenumbering{arabic}
%\setcounter{page}1
\thispagestyle{plain}
\begin{center}\textbf{\huge Preface}\end{center}{\huge \par}
\bigskip{}
%\singlespace
%\vspace{0.5cm}
Classical mathematical modelling is an art of expressing physical phenomena arise in nature (such as weather, biological processes, wave propagation, electromagnetic pulses etc.) into tractable mathematical formulations. These formulations are mainly concerned with the derivation and qualitative analysis of ordinary and partial differential equations, which give insight to the originating application. Conventionally these models are deterministic, i.e., all the necessary data to predict the solutions are available. On the contrary, the solution of a stochastic differential equation is though governed by these data, but not predetermined by them. 

In several instances, the physical systems experience external forcing. Usually these forcing factors are random in nature. Therefore, mathematical models need to be reformed in order to associate randomness in the system. This is the motivation behind studying stochastic partial differential equations (briefly SPDEs), which often yield more realistic models to predict these natural phenomena. Over the past few decades, the study of SPDEs has had an intensive development in pure and applied mathematics,  fluid mechanics, geophysics, theoretical physics etc.

The study of SPDEs not only helps in understanding these complex systems but also asks questions about the existence and uniqueness of various type of solutions and their statistical properties (e.g. invariant measures, ergodic behaviour, stability, large deviations principles etc). In this thesis we aim to study certain stochastic geometric partial differential equations (SGPDEs), namely,\\
(I) Nematic liquid crystals model, \\
(II) Navier-Stokes equations with constrained energy, \\
(III) Landau-Lifshitz-Gilbert equations. \\
Usual techniques for the analysis of SPDEs do not directly apply to our models in the conventional way due to the geometric nature of the problems. We prove existence of weak martingale solution in two and three dimensions for nematic liquid crystal (briefly NLC) model driven by pure jump noise in the Marcus canonical form. Moreover, we prove existence of a pathwise unique strong solution in two dimensions. Then we establish large deviation principle (LDP) for the law of the solutions of the NLC model perturbed by multiplicative Gaussian noise. This result on LDP is not straightforward to extend to the jump noise case, possibly due the (Marcus canonical) nature  of the noise and the need for the solution of the limiting  equation to stay on the unit sphere. Therefore we proceed in two steps. First, we consider the constrained  energy Navier-Stokes equation, which has structural similarity with the director field equation of the NLC, and study the LDP (in two spatial dimensions) in the presence of jump noise in the Marcus form. In the second step, we go to the coupled problem, i.e. the NLC model and make use of the techniques developed in the first step to establish LDP for the law of the solution of NLC model. Finally, we consider two-dimensional Landau-Lifshitz-Gilbert equations, which arise in the theory of magnetisation of ferromagnetic materials below Curie temperature and the constraint arise from the physical ``saturation" property of material. We are interested in special class of global strong solutions, which is uniquely characterised by the \index{forward bubbling property} ``forward bubbling" property. These kind of solutions has been introduced first by Struwe, where he studied the equation of heat flow of harmonic maps. We refer to these solutions as ``Struwe solutions". 

One of the major findings of the thesis is the study of ``Marcus canonical equation" in the context of SPDEs/SGPDEs, while proving existence and uniqueness results and establishing large deviation theory of the proposed problems. The It\^o formula remains as a major tool in the study of SPDEs. It has been observed that the usual integration by parts is not applicable for the It\^o formula and it fails to serve the usual chain rule (Newton-Leibniz type) of differential calculus. If we consider SPDEs and corresponding flows on smooth manifolds then the It\^o integral is not invariant under local coordinate transformation and so is not a crude geometric entity. In that case, we employ integral in the Stratonovich sense as perturbation of the It\^o integral, which can be treated according to the conventional rules of integration. However, these properties of Stratonovich integral are breached if the driving process has jumps. The work of Markus (subsequently by Applebaum, Kunita etc.) gives a headway in this direction, which is particularly very important in the contexts of SGPDEs. \\

A brief sketch of the chapter-wise content of the thesis is outlined below:
\begin{enumerate}
\item[(I)] {\bf Chapter 1. Introduction:}\\ In the introduction chapter, we provide the motivation behind studying deterministic and stochastic constrained partial differential equations and concisely sketch the relevant existing results that are available in the literature. We finish this chapter by discussing Marcus canonical form for stochastic differential equations perturbed by L\'evy noise.
\item[(II)] {\bf Chapter 2. Preliminaries:}\\ In the preliminaries chapter, we provide important definitions such as time homogeneous Poisson random measure. We define various functional spaces and state Aldous condition and Skorokhod representation theorems. We end the chapter by discussing about linear parabolic systems of general form. 
\item[(III)] {\bf Chapter 3. Stochastic Nematic Liquid Crystal model - Existence theory:}\\
In this chapter, we study the evolution equation which describes the system governing nematic liquid crystals, where the velocity equation is coupled with the director field equation. This system of equations are the Ginzburg-Landau approximation of the well-known Ericksen-Leslie equations. We study a physically relevant stochastic version of the system driven by pure jump noise (in the Marcus canonical form).  We prove the existence of a weak martingale solution for both two and three spatial dimensions. For the construction of the solution, we use a modified Faedo-Galerkin method based on the Littlewood-Paley decomposition. We employ the compactness method and the Jakubowski version of the Skorokhod representation theorem for non-metric spaces. For showing the tightness of laws of solutions, Aldous condition has been used. Moreover, we prove that  the martingale solution is pathwise unique in two dimensions. Then we use the infinite-dimensional version of the Yamada-Watanabe theory to deduce the existence of a strong solution as well. 
\item[(IV)] {\bf Chapter 4. The Large Deviation Principle - With Multiplicative Gaussian Noise:}\\
In this chapter, we consider the two dimensional stochastic nematic liquid crystal model perturbed by Gaussian noise. The noise is multiplicative Gaussian and is incorporated in the It\^o sense in the velocity equation and in the Stratonovich sense in the director field equation. We prove the Wentzell-Freidlin type large deviations principle (LDP) for the small noise asymptotic of solutions using weak convergence method. Based on the LDP developed in this work, we will be able to study the probability of switching of the director from the vicinity of one stationary solution to the another one and prove that the lower bound of the switching probability is strictly positive. This result might give a mathematical justification for a well-known physical phenomena called \index{Fr\'eedericksz transition} Fr\'eedericksz transition. Thus, this work may be viewed as an important step towards the understanding of director reversal phenomena, which we propose to take further in a subsequent work.
\item[(V)] {\bf Chapter 5. The Large Deviation Principle - With Jump noise in Marcus Canonical form:}\\
In this chapter, we study two problems (namely, Navier-Stokes equations (NSEs) with constrained energy and nematic liquid crystal (NLC) model). Since NSEs is a subsystem of NLC model, studying the NSEs with jump noise in Marcus form helps in understanding the behaviour of velocity equation of NLC model. 
\begin{enumerate}
\item
In the first part of the chapter, we consider the two dimensional stochastic constrained Navier-Stokes equations driven by L\'evy noise in the Marcus canonical form. At  first we prove the existence of a martingale solution based on the construction relying on classical Faedo-Galerkin approximations, compactness method and the Jakubowski's version of Skorokhod representation theorem for non-metric spaces. We further prove that the martingale solution is pathwise unique and deduce the existence of a strong solution. Then we establish a Wentzell-Freidlin type LDP for the small noise asymptotic of solutions using weak convergence method.
\item
Second part of this chapter is devoted to the establishment of Wentzell-Freidlin type LDP of nematic liquid crystals perturbed by pure jump noise in Marcus canonical form. As before, this work may be viewed as an important step towards the understanding of director reversal phenomena, which we propose to take further in a subsequent work.
\end{enumerate}
\item[(VI)] {\bf Chapter 6. Struwe like solutions for Stochastic Landau-Lifshitz-Gilbert Equations in two dimensions:}\\
In this chapter, we consider the Landau-Lifshitz-Gilbert equations (LLGEs) which describes the behaviour of the magnetisation in a ferromagnetic materials. This equation has structural similarity with the director field equation of the Ericksen-Leslie equation for NLC and also with harmonic map flow equation. The aim of this work is to prove the existence of a unique global strong (in the sense of both PDEs and probabilistic) solutions to the stochastic LLGEs (in Stratonovich sense), which is a standing open question. Such solutions should be ``regular" except for a singular set with finite number of singularities. For this, we employ the so called  Doss-Sussmann transformation in order to convert the stochastic system into a family of deterministic time dependent LLGE-like equation with random coefficients, and study this problem using the classical quasilinear PDE theory to prove the existence of maximal local strong  solution. Finally, using the reverse Doss-Sussmann transformation, we prove the equivalence of solutions of the transformed and the original problems, and then show that the solution is uniquely characterised by the ``forward bubbling" property. We conclude this chapter with some questions that we are currently working on.
\item[(VI)] {\bf Chapter 7. Concluding Remarks and Open Questions in Future Directions:}
In the final chapter of my thesis, we outline briefly the results obtained in the previous chapters. Then we end the chapter by framing some open questions related to the aforementioned problems. 
\end{enumerate}


%------------------------------------------------------------------------------
\cleardoublepage

